Reverse Modeling in Large Language Models

Humans are accustomed to reading and writing in a forward manner, and this natural bias extends to text understanding in auto-regressive large language models (LLMs). This paper investigates whether LLMs, like humans, struggle with reverse modeling, specifically with reversed text inputs. We found that publicly available pre-trained LLMs cannot understand such inputs. However, LLMs trained from scratch with both forward and reverse texts can understand them equally well during inference across multiple languages. Our case study shows that different-content texts result in different losses if input (to LLMs) in different directions -- some get lower losses for forward while some for reverse. This leads us to a simple and nice solution for data selection based on the loss differences between forward and reverse directions. Using our selected data in continued pretraining can boost LLMs' performance by a large margin across different language understanding benchmarks.

==> figures/step_loss_combine.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]
        \centering
        \includegraphics[width=0.48\textwidth]{figures/step_loss_change_norm.pdf}
        % \caption{Caption for Figure 1}
        \label{fig:step_loss_all}
    \end{subfigure}

    % \hfill
    % \vspace{1em}
    
    \begin{subfigure}[zzz]
        \centering
        \includegraphics[width=0.48\textwidth]{figures/step_loss_change_split_norm.pdf}
        % \caption{Caption for Figure 2}
        \label{fig:step_loss_split}
    \end{subfigure}
    \caption{Combined caption for both figures}
    \label{fig:step_loss_combine}
\end{figure}

==> tables/more_cases_ar.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\begin{tabularx}{\textwidth}{cXXXX}
\toprule
\textbf{Language} & \textbf{Texts Favoring Reverse (Low Reverse Loss)} & \textbf{Translation} & \textbf{Texts Favoring Forward (Low Forward Loss)} & \textbf{Translation} \\
\midrule
\multirow{1}{*}[-43em]{Arabic}
&
\begin{arabtext}
"بواسطة sbo-editor آخر تحديث الثلاثاء، 10 مارس 2015
صرح الممثل شون بين بأنه لن يعتذر إطلاقا عن تعليقه الساخر في حفل جوائز الأوسكار الذي واجه هجوما بسببه و ذلك عندما قال عن المخرج المكسيكي آليخاندرو غونزاليس إيناريتو ” من الذي أعطى لهذا اللعين الغرين كارد” و ذلك خلال تقديمه لجائزة أفضل فيلم سينمائي والتي فاز بها المكسيكي عن فيلمBirdman الذان عملا سويا في فيلم 21 Grams.
شون قال خلال الحملة الترويجية لفيلمه الجديد Gunman بأنه يتعجب من الإنتقادات المتكررة رغم تأكيده على أن آليخاندو هو إحدى أهم صانعي الأفلام في أمريكا و هذا التعليق لم يحمل أي نوايا عنصرية وغايته فقط هي إثارة الضحكات.
يذكر أن الثنائي بين وغونزاليس قد عملا معا من قبل في فيلم 21 Grams و قد صرح المخرج المكسيكي مباشرة عقب حفل الأوسكار أن هناك علاقة صداقة وطيدة تجمعه مع الممثل لذا هو يتقبل هذا التعليق بصدر رحب ويعتبرها مزحة مضحكة جدا.
Birdmanأليخاندرو غونزاليس أناريتوشون بين"
\end{arabtext}
& ``By sbo-editor last updated Tuesday, March 10, 2015
Actor Sean Penn said that he will never apologize for his sarcastic comment at the Academy Awards, for which he faced attacks, when he said about Mexican director Alejandro Gonzalez Inarritu, ``Who gave this motherfucker the green card?'' during his presentation of the award for Best Motion Picture, which the Mexican won. About the movie Birdman, they worked together in the movie 21 Grams.
Sean said during the promotional campaign for his new movie, Gunman, that he is surprised by the repeated criticism, despite his assertion that Alejando is one of the most important filmmakers in America. This comment did not carry any racist intentions and was only intended to provoke laughter.
It is noteworthy that the duo, Ben and Gonzalez, had previously worked together in the film 21 Grams, and the Mexican director stated immediately after the Oscar ceremony that there is a close friendship between him and the actor, so he accepts this comment with open arms and considers it a very funny joke.
Birdman Alejandro Gonzalez Anaritoshon Bea''
& 
\begin{arabtext}
إشتر عطر شانيل ألور سنشوال للنساء أو دي برفيوم - 100 مل أونلاين - إيزي كليك
شانيل الور سنشوال عطر نسائي راقي، رائحته شرقية زهرية جميلة وساحرة، عبيره فواح وقوي الثبات ويضيف لمسات أنيقة ملفتة للأنظار ولا تقاوم وتدوم لفترات طويلة. انظر الوصف لمزيد من المعلومات
شانيل الور سنشوال عطر نسائي راقي، رائحته شرقية زهرية جميلة وساحرة، عبيره فواح وقوي الثبات ويضيف لمسات أنيقة ملفتة للأنظار ولا تقاوم وتدوم لفترات طويلة.
أطلقته شانيل عام 2005 ويعتبر من أهم الإصدارات ويمتاز برائحة ساحرة مفعمة بالحيوية وتعطي إحساس بالنعومة والدفء ويأتي عطر شانيل الور سنشوال في زجاجة شفافة مستطيلة الشكل 100 مل وبغطاء معدن نبيتي اللون فيضفي جمالا وسحرا على لون العطر، وتركيزه أو دي برفيوم، ويتكون من:
مقدمة العطر: مقدمة العطر : البرغموت والباتشولي واليوسفي والفلفل الوردي
قلب العطر: قلب العطر : زهور السوسن والياسمين والورد وفواكه مجففة
قاعدة العطر: قاعدة العطر : التوابل والأخشاب ونجيل الهند والفانيليا والعنبر
يتميز عطر شانيل الور سنشوال برائحة ساحرة ورقيقة تضفي جمالا للمرأة ويعكس أناقتها وأنوثتها فيفتتح العطر رائحة الحمضيات المنعشة و ينقلنا بسلاسة ونعومة لقلب من الزهور والفواكه ويختم بالأخشاب والعنبر والفانيليا فترسم هالة من الروائح الخيالية الساحرة ويتم استخدامه في جميع الأوقات والمناسبات."
\end{arabtext}
& Buy Chanel Allure Sensual for Women Eau de Parfum - 100 ml online - Easy Click
Chanel Allure Sensual is a sophisticated women's perfume. It has a beautiful and charming oriental floral scent. Its fragrance is fragrant and has a strong consistency. It adds elegant touches that catch the eye and are irresistible and last for long periods. See description for more information
Chanel Allure Sensual is a sophisticated women's perfume. It has a beautiful and charming oriental floral scent. Its fragrance is fragrant and has a strong consistency. It adds elegant touches that catch the eye and are irresistible and last for long periods.
It was launched by Chanel in 2005 and is considered one of the most important releases. It is characterized by a charming, lively scent that gives a feeling of softness and warmth. Chanel Allure Sensual perfume comes in a 100 ml transparent rectangular bottle with a burgundy metal cap, adding beauty and charm to the color of the perfume, and its concentration as eau de parfum. It consists of:
Top notes: Top notes: bergamot, patchouli, mandarin, and pink pepper
Heart of perfume: Heart of perfume: iris, jasmine, rose and dried fruits
Base notes: Base notes: spices, woods, vetiver, vanilla and amber
Chanel Allure Sensual perfume is characterized by a charming and delicate scent that adds beauty to a woman and reflects her elegance and femininity. The fragrance opens with a refreshing citrus scent and transports us smoothly and softly to a heart of flowers and fruits. It concludes with woods, amber and vanilla, creating an aura of enchanting imaginative scents. It is used at all times and occasions.\\
\bottomrule
\end{tabularx}
\caption{Case study in Arabic. Included are both the original German texts and their English translations.}
\label{tab:more_cases_ar}
\end{table*}

==> tables/more_cases_ko.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\begin{tabularx}{\textwidth}{cXXXX}
\toprule
\textbf{Language} & \textbf{Texts Favoring Reverse (Low Reverse Loss)} & \textbf{Translation} & \textbf{Texts Favoring Forward (Low Forward Loss)} & \textbf{Translation} \\
\midrule
\multirow{1}{*}[-40em]{Korean} & 
"미국 동영상 서비스 시장, 최종 승자는 누구? - B2B IT 전문가 진행 생방송토크 웨비나
전 세계에서 인터넷 동영상 서비스(Over The Top, OTT) 경쟁이 한창이다. 글로벌 온라인 동영상 스트리밍 서비스의 선두주자 넷플릭스, 아마존닷컴의 인터넷 주문형 동영상 서비스 아마존 비디오, 동영상 공유 사이트 유튜브 등 각자의 서비스를 내세우며 피 터지는 경쟁을 하고 있다. 중심지는 아무래도 미국이다. 글로벌 IT기업의 집결지인 미국 무대를 먼저 사로잡아야 전 세계 고객들을 사로잡을 수 있다는 생각으로 오리지널 콘텐츠 개발 등 각종 공격적 마케팅 전략을 쏟아내고 있다.
콘텐츠 개발을 위한 투자 예산도 어마어마하다. 지난 4월7일 <비즈니스인사이더> 보도에 따르면, 아마존이 2017년 동영상 서비스 강화를 위해 투입할 예산이 45억달러, 우리 돈 5조1천억원 규모라는 JP모건 애널리스트들의 분석이 나왔다. 브라이언 올사브스키 아마존 CFO 역시 “아마존 비디오에 대한 투자를 두 배 가까이 늘릴 것”이라고 말한 바 있다. 넷플릭스도 만만치 않다. 넷플릭스는 지난해 말, 2017년 서비스 강화를 위해 50억달러, 우리돈 5조7천억원 규모를 투입할 예정이라고 말했다. 두 회사의 투자 규모만 합쳐도 우리돈 12조원 정도 예산이니 가히 엄청나다고 할 수 있다.
(자료=컴스코어)
미국 인터넷 시장조사 연구기업 컴스코어가 OTT 서비스 시장에 대한 조사 보고서를 4월10일 내놓았다. 컴스코어에 따르면, 2016년 12월을 기준으로 미국 내에 인터넷 연결망을 가진 가구 중 53\%인 약 4900만 가구가 인터넷 동영상 서비스에 가입했다고 한다. 단순히 가입 규모에 그치지 않는다. 이들의 전체 평균 시청 시간은 월 평균 19일, 일 평균 2.2시간이다. 현재 미국인들의 하루 평균 TV 시청 시간은 4시간 수준이다. 케이블 위성 방송으로만 TV를 시청하던 전통적인 시청 패턴이 완전히 변화하고 있음을 알 수 있다. ... 
& "US video service market, who will be the final winner? - Live talk webinar hosted by B2B IT experts
Competition in Internet video services (Over The Top, OTT) is in full swing around the world. Netflix, the leader in global online video streaming services, Amazon.com's Internet video-on-demand service Amazon Video, and video sharing site YouTube are competing fiercely by offering their own services. The center is obviously the United States. They are pouring out various aggressive marketing strategies, including the development of original content, with the belief that they can captivate customers around the world only by capturing the American stage, the gathering place of global IT companies, first.
The investment budget for content development is also enormous. According to a report by <Business Insider> on April 7, JP Morgan analysts analyzed that Amazon's budget to invest in strengthening video services in 2017 is \$4.5 billion, or 5.1 trillion won. Amazon CFO Brian Olsavsky also said, “We will nearly double our investment in Amazon Video.” Netflix is no slouch either. Netflix said at the end of last year that it plans to invest \$5 billion, or 5.7 trillion won, to strengthen its services in 2017. The combined investment size of the two companies alone amounts to a budget of approximately 12 trillion won, which can be said to be truly enormous.
(Data = ComScore)
ComScore, an American internet market research company, released a research report on the OTT service market on April 10. According to ComScore, as of December 2016, approximately 49 million households, or 53\% of households with an Internet connection in the United States, had subscribed to Internet video services. It’s not just about the size of subscriptions. Their overall average viewing time is an average of 19 days per month and 2.2 hours per day. Currently, the average amount of time Americans watch TV per day is around 4 hours. It can be seen that the traditional viewing pattern of watching TV only through cable and satellite broadcasting is completely changing. ...
& "[37\% 세일] Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 쿠폰 코드 인기 쿠폰, Jul 2020 - iVoicesoft
인기 쿠폰 › Cdkeys 쿠폰 코드 2020 › Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 쿠폰의 할인 할인 코드 37\% 세일, 여름 제공
간단히 버튼을 클릭하십시오 [할인 된 가격으로 즉시 구매] 쿠폰을 사용하려면 37\% 할인 코드. 쿠폰 코드가 포함되었습니다. 결제시 코드를 입력하십시오.
특별승진의 ($16.42 절약)$16.42 절약
여름 은 위대하 Cdkeys 제공 받기에 완벽한시기입니다. 2020 년 여름 제공 위해 지금 청구하십시오. 현재 거래: 37\% 할인 Star Wars Battlefront II 2 - Celebration Edition Xbox One (US). Cdkeys 에서 원하는 것을 가져올 수있는 최고의 기회. 제한된 시간 동안 만. 결제시 코드를 입력하십시오.
Cdkeys 쿠폰 코드: 최고의 세일즈 프로모션 사용하여 매력적인 가격으로 훌륭한 제품을 찾으십시오. 37\% 할인 Star Wars Battlefront II 2 - Celebration Edition Xbox One (US), 16.42 절약. 쇼핑하려면 클릭하세요. 제한된 시간 동안 만.
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)에 대하여
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)소개
Get 37\% OFF of Star Wars Battlefront II 2 - Celebration Edition Xbox One (US), a 위대하 in 여름 제공
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 쿠폰 코드. Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 위대하 여름 제공 37\% 쿠폰 코드.
왜 우리의 Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 쿠폰 코드를 적용해야합니까?
간단 해! 최신 Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 프로모션 코드를 수집하여 제공했습니다, 가장 큰 할인으로. 또한 모든 Cdkeys 제품에 대한 최고의 절감 효과를 제공합니다.
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) 할인 코드에 대한 의견" 
& "[37\% Sale] Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) Coupon Code Popular Coupons, Jul 2020 - iVoicesoft
Popular Coupons › Cdkeys Coupon Codes 2020 › Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) Coupon Discount Discount Code 37\% Sale, Summer Offer
Simply click the button [Buy Instantly at Discounted Price] to use coupon 37\% discount code. Coupon code included. Enter code at checkout.
Special Promotion (Save \$16.42)Save \$16.42
Summer is the perfect time to get great Cdkeys offers. Claim now for summer 2020 offer. Current deal: 37\% off Star Wars Battlefront II 2 - Celebration Edition Xbox One (US). Best chance to get what you want from Cdkeys. Only for a limited time. Enter code at checkout.
Cdkeys Coupon Code: Find great products at attractive prices using our best sales promotions. 37\% off Star Wars Battlefront II 2 - Celebration Edition Xbox One (US), saving 16.42. Click to shop. For a limited time only.
About Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US)Introduction
Get 37\% OFF of Star Wars Battlefront II 2 - Celebration Edition Xbox One (US), a great offer in summer
Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) Coupon Code. Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) Greatest Summer Offer 37\% Coupon Code.
Why apply our Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) coupon code?
It's simple! We have collected and provided you with the latest Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) promo codes, with the biggest discounts. We also offer the best savings on all Cdkeys products.
Opinions on Star Wars Battlefront II 2 - Celebration Edition Xbox One (US) Discount Code"
\\
\bottomrule
\end{tabularx}
\caption{Case study in Korean. Included are both the original Korean texts and their English translations.}
\label{tab:more_cases_ko}
\end{table*}
